Maximin Optimization for Binary Regression

We consider regression problems with binary weights. Such optimization problems are ubiquitous in quantized learning models and digital communication systems. A natural approach is to optimize the corresponding Lagrangian using variants of the gradient ascent-descent method. Such maximin techniques are still poorly understood even in the concave-convex case. The non-convex binary constraints may lead to spurious local minima. Interestingly, we prove that this approach is optimal in linear regression with low noise conditions as well as robust regression with a small number of outliers. Practically, the method also performs well in regression with cross entropy loss, as well as non-convex multi-layer neural networks. Taken together our approach highlights the potential of saddle-point optimization for learning constrained models.

==> content/related.tex <==
\section{Related Work}
\subsection{Quantized Networks:}
The BinaryConnect method \cite{binaryConnect} was the first to propose the idea of straight-through estimation for optimizing with the sign function. This was later extended to more general low-precision weights and activations \citep{Hubara:2017:QNN}. Although sometime empirically successful, there is no theoretical justification for using straight-through estimation. As we argue above, on one hand STE is not a descent direction in the binary linear regression case (see supplementary material), and indeed in our experiments it does perform as well as our proposed maximin approach. The only theoretical account of STE is in \cite{yin2019understanding} who do not analyze binarized weights, but rather the case of a binary activation function, and also under the assumption of Gaussian inputs.  


STE and variants are sometime presented as having regularization effects due to the binarization step. Our work introduces an explicit regularizer and, importantly, learns the regularizer coefficients for all weights. Some earlier works have introduced regularization, but with one coefficient for the entire model, which is significantly weaker than our approach, and lacks theoretical support. For example, \cite{choi2018learning,tang2017train} proposed adding a quadratic regularizer $(1-w^2)$ but had a single coefficient for all weights, and did not train it. A variant of this regularizer was also explored in \cite{darabi2018bnn+}. In the context of binary compressed sensing, \cite{fosson2018non} proposed quadratic regularization  (see also \cite{fosson2019recovery}). Regularization for multi-level quantization was proposed in \cite{choi2018learning}.

Most advanced quantization schemes employ STE to optimize with non-differentiable quantization operations. For example \cite{XNOR} uses STE to binarize activations in addition to the weights and \cite{dorefaNet} also quantizes the gradients using stochastic STE. \cite{bethge2019back} summarizes recent efforts and introduces a list of common practices for quantizing networks using STE. Finally, \cite{BNN_gumbelSoftmax} proposed to address the discrete aspect of the problem via the Gumble softmax trick, but also uses STE in the optimization. 
%an alternative to STE that samples from approximated differential distribution using the Gumbel softmax trick, the drawback is obviously the continious nature of the sampled weights, which they propose to solve with a vaiant of STE.


\subsection{Saddle Point Optimization}
Our approach is to use the dual formulation of the original constrained problem, and arrive at a maxmin optimization problem of its Lagrangian. This approach has been considered before in \cite{eban2016large} for handling ranking based objectives, and in \cite{nandwani2019primal} for imposing natural constraints over the
output label space. These are all instances of the saddle-point optimizations. Such problems have attracted considerable interest in machine learning recently, due to the fact that GAN training is a saddle-point problem. In particular, one would like to understand when first order optimization methods (such as gradient descent-ascent, or extra-gradient) will converge to a local or global saddle-point \cite{localMinimax,daskalakis2018limit,gidel2016frank,heusel2017gans}. As in standard minimization problems it turns out that first order methods will converge to global saddle-points (i.e., ones that solve the maxmin problem) if there are no local saddle-points.  There are however multiple subtleties for the saddle-point case, as shown in \cite{localMinimax}. 

Our results demonstrate one of the first cases where the maxmin problem is not concave-convex, yet convergence of first order methods to the global solution is guaranteed. 
